On the Hardness of Robust Classification

It is becoming increasingly important to understand the vulnerability of machine learning models to adversarial attacks. In this paper we study the feasibility of robust learning from the perspective of computational learning theory, considering both sample and computational complexity. In particular, our definition of robust learnability requires polynomial sample complexity. We start with two negative results. We show that no non-trivial concept class can be robustly learned in the distribution-free setting against an adversary who can perturb just a single input bit. We show moreover that the class of monotone conjunctions cannot be robustly learned under the uniform distribution against an adversary who can perturb $\omega(\log n)$ input bits. However if the adversary is restricted to perturbing $O(\log n)$ bits, then the class of monotone conjunctions can be robustly learned with respect to a general class of distributions (that includes the uniform distribution). Finally, we provide a simple proof of the computational hardness of robust learning on the boolean hypercube. Unlike previous results of this nature, our result does not rely on another computational model (e.g. the statistical query model) nor on any hardness assumption other than the existence of a hard learning problem in the PAC framework.

==> sections/rob-less2.tex <==
In the standard PAC framework a hypothesis $h$ would be considered to
have zero risk with respect to a target concept $c$ if $\Pr{x\sim
D}{h(x)\neq c(x))=0$.  We have remarked that exact learnability
implies robust learnability; we next give an example of a
concept that that is PAC learnable with zero risk but yet cannot be
robustly learned (regardless of the sample complexity).

We next observe that the class of dictators
(i.e., conjunctions of length one) can be learned in the standard PAC
model with zero risk but yet cannot be robustly learned (regardless of
the number of samples): 



\paragraph{Sample Complexity under Distributional Assumptions} 
The impossibility of robust learning in the distribution-free setting
stems from the fact that the dependence of a target concept on a
particular feature can be hidden from the learner if the distribution
over examples is sufficiently biased.  While this is not an obstacle
for PAC learnability, this hidden dependence can be exploited in the
adversarial setting.  This leads us to identify assumptions that
exclude such biased distributions.  We proceed to study robust
learnability of the class of monotone conjunctions under such
distributional assumptions.  We focus on monotone conjunctions because
the dependence of concepts on features is particularly simple and
transparent for this class.  Here we show that robust learning with
polynomial sample complexity is possible against an adversary who can
perturb $O(\log n)$ bits.  We show moreover that this bound is tight:
robust learning is impossible, even under the uniform distribution,
against an adversary who can perturb a superlogarithmic number of
bits.

\paragraph{Computational Complexity}

The work that is most directly related to this paper
is~\cite{diochnos2018adversarial}, which considers the robustness of
monotone conjunctions under the uniform distribution on the boolean
hypercube.  In particular~\cite[Section 4]{diochnos2018adversarial}
considers a notion of \emph{error region} loss, which concides with
the \emph{exact-in-the-ball} loss that is our main focus.
However~\cite{diochnos2018adversarial} do not address the sample and
computational complexity of learning: their results rather concern the
ability of an adversary to magnify the missclassification error of
\emph{any} hypothesis with respect to \emph{any} target function by
perturbing bits of the input.  For example, they show that an
adversary who can perturb $O(\sqrt{n})$ bits can increase the
missclassification probability from $0.01$ to $1/2$.  By contrast we
show that a weaker adversary, who can perturb only $\omega(\log n)$
bits, makes it impossible to learn monotone conjunctions with
polynomial sample complexity.  The main tool used
in~\cite{diochnos2018adversarial} is the isoperimetric inequality for
the Boolean hypercube, which gives lower bounds on the volume of the
expansions of arbitrary subsets.  On the other hand, we use the
probabilistic method to establish the existence of a single hard to
learn target concept for any given algorithm with polynomial sample
complexity.




\section{Definition of Robust Learning}

\subsection{Choosing a Robust Loss Function}
The notion of robustness can be accommodated within the basic set-up
of PAC learning by adapting the definition of loss function.  In this
section we review two of the main definitions of \emph{robust loss}
that have been used in the literature.  For concreteness we consider
an input space $\mathcal{X}=\{0,1\}^n$ equipped with Hamming distance
as a metric $d:\mathcal{X}\times\mathcal{X}\rightarrow\mathbb{N}$.
Given $x\in\mathcal{X}$, we write $B_\rho(x)$ for the ball $\{y\in
\mathcal{X} : d(x,y)\leq \rho\}$ with centre $x$ and radius $\rho\geq
0$.

The first definition of robust loss asks that the hypothesis $h$ be
exactly equal to the target concept $c$ in the ball $B_\rho(x)$ of
radius $\rho$ around a ``test point'' $x\in\mathcal{X}$:
\begin{definition}
\label{def:loss-correct}
Given respective hypothesis and target functions
$h,c:\mathcal{X}\rightarrow\{0,1\}$, distribution $D$ on
$\mathcal{X}$, and robustness parameter $\rho\geq 0$, we define the
``exact in the ball'' robust loss of $h$ with respect to $c$ as
\begin{equation*}
\roblosse(h,c)=\Pr{x\sim D}{\exists z\in B_\rho(x):h(z)\neq c(z)}
\enspace.
\end{equation*}
\end{definition}
The robustness parameter captures the power of an adversary who can
alter at most $\rho$ bits of the input.  Then the robust loss is the
probabilty that a point sampled from distribution $D$ can be altered
by such an adversary so as to cause a missclassification.  Note that
if $h=c$ then $h$ incurs robust loss zero.

While this definition captures a natural notion of robustness,
evaluating the loss function requires that the learner have knowledge
of the target function outside of the training set, e.g., through
membership queries.  Nonetheless, by considering a learner who has
oracle access to the predicate ${\exists z\in B_\rho(x):h(z)\neq
  c(z)}$, we can use the exact-in-the-ball framework to analyse 
sample complexity and to prove strong lower bounds
on the computational complexity of robust learning.

A popular alternative to the exact-in-the-ball loss function in
Definition~\ref{def:loss-correct} is the following
\emph{constant-in-the-ball loss} function:
\begin{definition}
\label{def:loss-constant}
Given respective hypothesis and target functions
$h,c:\mathcal{X}\rightarrow\{0,1\}$, distribution $D$ on
$\mathcal{X}$, and robustness parameter $\rho\geq 0$, we define the
``constant in the ball'' robust loss of $h$ with respect to $c$ as
\begin{equation*}
\roblossc(h,c)=\Pr{x\sim D}{\exists z\in B_\rho(x):h(z)\neq c(x)}
\enspace.
\end{equation*}
\end{definition}

The obvious advantage of Definition~\ref{def:loss-constant} over
Definition~\ref{def:loss-correct} is that in the former definition,
evelauting the loss at point $x\in\mathcal{X}$ requires only knowledge
of the correct label of $x$ and the hypothesis $h$.  In particular,
this definition can also be carried over to the non-realizable
setting, in which there is no target.  However from a foundational
point of view the constant-in-the-ball loss function fails some basic
sanity checks.  Under this definition it is possible to have strictly
positive robust loss in the case that $h=c$: if the $\rho$-expansion
of the decision boundary (i.e., the space of all points within a
distance $\rho$ of the boundary) has positive probability, any point
in that region will have loss of~1.  Additionally, when we work in the
hypercube, or a bounded input space, as $\rho$ becomes larger, we
eventually require the function to be constant in the whole space.
Essentially, to $\rho$-robustly learn in the realisable setting, we
require concept and distribution pairs to be represented as two sets
$D_+$ and $D_-$ whose $\rho$-expansions don't intersect, as
illustrated in Figures~1 and 2.  These limitations appear even more
stringent when we consider simple concept classes such as parity
functions, which are defined for an index set $I\subseteq [n]$ as
$f_I(x)=\sum_i x_i\mod 2$.  This class can be PAC-learned, as well as
exactly learned with $n$ membership queries.  However, for any point,
it suffices to flip one bit of the index set to switch the label, so
$\roblossc(f_I,f_I)=1$ for any $\rho\geq1$.

Ultimately, we want the adversary's power to come from creating
perturbations that cause the hypothesis and target functions to differ
in some regions of the input space.  For this reason we favour the
exact-in-the-ball definition and henceforth work with that.

Having settled on a loss function, we now formulate the definition of
robust learning.  For our purposes a \emph{concept class} is a family
$\mathcal{C} = \{\mathcal{C}_n\}_{n\in \mathbb{N}}$, with
$\mathcal{C}_n \subseteq \{0,1\}^{\{0,1\}^n}$.  Likewise a
\emph{distribution class} is a family $\mathcal{D} = \{
\mathcal{D}_n\}_{n\in\mathbb{N}}$, with $\mathcal{D}_n$ a set of
distributions on $\{0,1\}^n$.  Finally a \emph{robustness function} is
a function $\rho:\mathbb{N}\rightarrow \mathbb{N}$.

\begin{definition}
\label{def:robust-learning} 
Fix a function $\rho:\N\rightarrow\R$. We say that an algorithm $\A$
\emph{efficiently} $\rho$-\emph{robustly learns} a concept class $\C$
with respect to distribution class $\mathcal{D}$ if there exists a
polynomial $\poly$ such that for all $n\in\mathbb{N}$, all target
concepts $c\in \C_n$, all distributions $D \in \mathcal{D}_n$, and all
accuracy and confidence parameters $\epsilon,\delta>0$, there exists
$m \leq \poly(1/\epsilon,1/\delta,n)$, such that when $\A$ is given
access to a sample $S\sim D^m$ it outputs
$h:\{0,1\}^n\rightarrow\{0,1\}$ such that $\Pr{S\sim
  D^m}{\ell^E_{\rho(n)}(h,c)<\epsilon}>1-\delta$.
\end{definition}

Note that the definition of robust learning requires polynomial sample
complexity and allows improper learning (the hypothesis $h$ need not
belong to the concept class $\mathcal{C}_n$).


We denote by $\X$ an input space  of dimension $n$ and by $\C\subseteq\set{0,1}^\X$ the concept class to be learned.
We get access to labelled data $S=\set{(x_i,c(x_i))}_{i=1}^m$, where $x_i\in\X$ and $c\in\C$.
Not only do we require that the hypothesis we learn be close to the concept that labelled the data, we also want to be \emph{robust} against an adversary that could perturb points in $\X$. 
Given a metric $d$ on $\X$ and a robustness parameter $\rho$, the adversary's power is limited by only allowing to perturb a point $x$ in the $\rho$-ball of radius $\rho$ centred at $x$, which we will denote $B_\rho(x)$.
In this work, the robustness parameter is a function $\rho:\N\rightarrow\R$ that depends on the dimension $n$ of $\X$, and we will drop the dependence on $n$ when it is clear from the context.

\begin{definition}[Efficient Robust Learning, Realizable Case]
\label{def:robust-learning} 
Fix a function $\rho:\N\rightarrow\R$. We say that an algorithm $\A$ \emph{efficiently} $\rho$-\emph{robustly learns} a concept class $\C$  with respect to 
%a distribution family $\D$ on $\X$ and 
a robust loss function $\robloss$ if there exists a polynomial $\poly$ such that for any target concept $c\in \C$, any distribution $D$ on $\X$, any accuracy and confidence parameters $\epsilon,\delta>0$, when $\A$ is given access to a sample $S\sim D^m$, where $m\geq\poly(1/\epsilon,1/\delta,\text{size}(c),d)$, $\A$ outputs $h\in \set{0,1}^\X$ such that $\Pr{S\sim D^m}{\robloss(h,c)<\epsilon}>1-\delta$.
\end{definition}

\qn{I could amend the definition to add robust learnability with respect to a family of distributions $\D$, as we later show that it's impossible to robustly learn in the distribution-free setting. I also added \emph{efficiently} to avoid any confusion. Thoughts? Should I highlight this?}

The definition above works for an arbitrary input space $\X$ and metric $d$.
However, for the rest of the paper and unless otherwise stated, we will be working on the boolean hypercube, i.e. $\X=\boolhc$, and use the Hamming distance as our metric $d$. 
This is one of the reasons that we require a sample complexity that is polynomial in the learning parameters, similarly to the PAC-learning setting (whose definition we can recover by setting $\rho=0$).
Indeed, it would suffice to wait long enough to see all the support of the distribution.
In this papr, we will then sometimes simply refer to robust learnability to mean \emph{efficient} robust learnability. 
It however might be more relevant to consider \emph{finite} sample complexity in other settings, for example in $\R^n$.

For now, we do not impose any restrictions on what kind of oracle we have access to in order to obtain a training sample $S$.
Finally, note that Definition~\ref{def:robust-learning} allows \emph{improper learning} (the algorithm does not need to output a hypothesis in $\C$) and is \emph{distribution-free}, in the sense that . 
In certain cases, we will consider \emph{distribution-dependent} robust learning algorithms, where the distribution from which we sample the data is fixed.

\subsection{Robust Loss Functions}

*Note: cite which papers used which loss function*

Two main definitions of robust loss have been used in the literature so far. 
As remarked later in this section, they each come with their own limitations and differ in their meaning of robustness.
Let us first consider what is arguably the most common of these functions, where we require the function that we have learned to be constant in a ball around a given point.

\begin{definition}[Robust Loss, Constant in the Ball] 
\label{def:loss-constant}
For $h,c\in\C$, $x\in\X$, $\rho\in\R_{\geq0}$, we define the ``constant in the ball'' robust loss as
\begin{equation*}
\roblossc(h,c)=\Pr{x\sim D}{\exists z\in B_\rho(x):h(z)\neq c(x)}
\enspace.
\end{equation*}
\end{definition}

This loss presents a practical advantage: 
its computation does not explicitly rely on access to membership queries.
Indeed, once we have sampled an example from the distribution at hand, we assume that all the examples in a ball centred at this example will share the same label. 
This definition also easily translates to the agnostic setting, where a target concept is not required. 

However, in the realisable setting, it is possible to have strictly positive robust loss in the case we have learned the target function: if the $\rho$-expansion of the decision boundary (i.e., the space of all points within a distance $\rho$ of the boundary) has positive probability, any point in that region will have loss of~1.
Additionally, when we work in the hypercube, or a bounded input space, as $\rho$ becomes larger, we eventually require the function to be constant in the whole space.
Essentially, to $\rho$-robustly learn in the realisable setting, we require concept and distribution pairs to be represented as two sets $D_+$ and $D_-$ whose $\rho$-expansions don't intersect, as illustrated in Figures~1 and 2.
These limitations appear even more stringent when we consider simple concept classes such as parity functions, which are defined for an index set $I\subseteq [n]$ as $f_I(x)=\sum_i x_i\mod 2$.
This class can be PAC-learned, as well as exactly learned with $n$ membership queries.
However, for any point, it suffices to flip one bit of the index set to switch the label, so $\roblossc(f_I,f_I)=1$ for any $\rho\geq1$. 

Ultimately, we would want the adversary's power to come from creating perturbations that cause the hypothesis and target functions to differ in some regions of the input space.
For these reasons, we might want to consider another loss function, where we require the hypothesis to be \emph{exact} in the ball centred at a point sampled from a given distribution. 

\begin{figure}
  \label{fig:constant}
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[scale=0.5]{imgs/constant-function}
  \caption{Robust learning requires the target to be constant in the support of the distribution.}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
  \includegraphics[scale=0.5]{imgs/disjoint-supports}
  \caption{The $\rho$-expansion of the support of the distribution allows non-trivial concepts to be robustly learned. }
\end{minipage}
\end{figure}


\begin{definition}[Robust Loss, Exact in the Ball] 
\label{def:loss-correct}
For $h,c\in\C$, $x\in\X$, $\rho\in\R_{\geq0}$, we define the ``exact in the ball'' robust loss as
\begin{equation*}
\roblosse(h,c)=\Pr{x\sim D}{\exists z\in B_\rho(x):h(z)\neq c(z)}
\enspace.
\end{equation*}
\end{definition}

In certain circumstances, this definition could be closer to the intended meaning of robust learning: if an adversary perturbs a point beyond the target's decision boundary, then the function we have learned should capture this change in label.
In this setting, it is theoretically possible to robustly learn with respect to a distribution $D$ even when the $\rho$-expansion of the support of $D$ is connected, as in Figure 1.
This gives examples where the ``exact in the ball'' robust loss is zero, while the ``constant in the ball'' one is non-zero with strictly positive probability.
But are there examples where the opposite happens?
Figure~3 gives such an example, where both functions have exactly learned in the sense of definition~\ref{def:exact-learning}, but where the $\roblossc=0$, while $\roblosse>0$.

\begin{figure}[b]
  \label{fig:diff-losses}
  \centering
%  \input{imgs/diff-losses}
	\includegraphics[scale=0.5]{imgs/diff-rob-losses}
	\caption{An example where the robust losses differ. The red concept is the target, while the blue one is the hypothesis. The blue points are the support of the distribution and the shaded region represents their $\rho$-expansion. The red points represent perturbed inputs.}
\end{figure}

\subsection{Relationship between Robust and Exact Learning}

Before going further, we might want to consider when exactly learning $\C$ implies that we have robustly learned $\C$ and vice-versa. 
By \emph{exactly learning}, we mean that, with high probability over the training sample, we return a hypothesis that is correct with probability 1, hence the term \emph{distribution-specific} exact learning.

\begin{definition}[Distribution-Specific Exact Learning]
\label{def:exact-learning} We say that an algorithm $\A$ \emph{exactly learns} a concept class $\C$ if for any target concept $c\in \C$ and any distribution $D$, $\A$ outputs $h\in \set{0,1}^\X$ such that $\Pr{x\sim D}{h(x)\neq c(x)}=0$ with probability at least $1-\delta$ .
\end{definition}

Note that we do not require the hypothesis to be correct outside the support of the distribution. 
This is a sensible concession: if we are trying to classify digits for example, we should not care about the label of an image whose pixels were generated at random.
From now on, we will refer to distribution-specific exact learning simply as exact learning, as it is the only definition we consider in this work.

\subsubsection{Exact Learning Does Not Imply Robust Learning}
\label{sec:dictators}

As previously mentioned, it is possible that, even in the case we learn the target concept, we have not robustly learned with respect to the ``constant in the ball'' definition of robust loss. 
The same argument clearly cannot be applied to Definition~\ref{def:loss-correct}.
However, while this latter definition seems natural, we can construct an example on the boolean hypercube where a very simple concept class is not robustly learnable by choosing two concepts that agree on the label of any point drawn at random from a specific distribution.

\begin{lemma}
\label{lemma:dictators}
The class of  dictators, i.e. the concept class where $c(x)$ only depends on one variable $x_i$ for $i\in[n]$, is not 1-robustly learnable (and thus not robustly learnable for any $\rho\geq1$) with respect to the robust loss of Definition~\ref{def:loss-correct}. 
\end{lemma}
\begin{proof}
%First observe that, when we get an example $(x, c(x))$ we know that any variable in $x$ that does not have the same value as $c(x)$ cannot be the dictator.
%Our strategy is to choose a distribution and concepts such that a training sample will look the same regardless of which concept labelled it.
Let $c_1$ and $c_2$ be the dictators on variables $x_1$ and $x_2$, respectively.
Let $D$ be such that $\Pr{x\sim D}{x_1=x_2}=1$ and $\Pr{x\sim D}{x_k=1}=\frac{1}{2}$
for $k\geq3$. 
Draw a sample $S\sim D^m$ and label it according to $c\sim U(c_1,c_2)$. 
By the choice of $D$, the elements of $S$ will have the same label regardless of whether $c_1$ or $c_2$ was picked.
However, for $x\sim D$, it suffices to flip any of the first two bits to cause $c_1$ and $c_2$ to disagree on the perturbed input.
We can easily show that, for any $h\in\set{0,1}^\X$, 
\begin{equation*}
 \ell^E_1(c_1,h)+ \ell^E_1(c_2,h)
\geq  \ell^E_1(c_1,c_2) = 1 \enspace.
\end{equation*}
Then 
\begin{equation*}
\underset{c\sim U(c_1,c_2)}{\mathbb{E}}\eval{S\sim D^m}{ \ell^E_1(h,c)} \geq 1/2 \enspace.
\end{equation*}
\end{proof}

As shown in this example, there are settings where distribution-specific exact learning as in Definition~\ref{def:exact-learning} does not imply robust learning. 
Picking any of $c_1$ or $c_2$ (or their conjunction) as our hypothesis will give us an expected loss of 0 with probability 1, but an adversary potentially just needs to change one bit of a random example to cause a label mismatch between the hypothesis and the target concept.

\begin{remark}
It could seem tempting to further restrict an adversary's power by only allowing perturbations that remain in the support of the distribution, as it is clear that exact learning implies robust learning in this setting.
However, we omit this definitions for two reasons.
First, it does not capture the way in which robust learning has been considered in the recent adversarial learning literature. 
For example, if an adversary perturbs the image of the digit 1, which was sampled from a ``natural'' distribution $D$, and changes a small number of pixels in the background, the resulting image is presumably not in the support of $D$, but should still be classified as a 1.
Second, it is always possible to circumvent the constraint that the adversary must remain in the support of the distribution by picking an insignificant fraction of the probability mass and uniformly distribute it outside of the support of the distribution. 
For these reasons, we will from now on mostly look at robust learning with respect to Definition~\ref{def:loss-correct}.
\end{remark}

\subsubsection{The Distribution-Dependent Setting}

We saw that, for both robust losses $\roblossc$ and $\roblosse$, exact learning does not necessarily imply robust learning. 
Moreover, as we will later show, efficient distribution-free robust learning is not possible (see Section~\ref{sec:no-dfrl}).
What if we have access to a robust learning algorithm for a specific distribution on the boolean hypercube?
In this section, we show that distribution-dependent robust learning implies distribution-dependent exact learning for both robust loss definitions, under certain conditions on the measure of balls in the support of the distribution.
Let us start with definition~\ref{def:loss-correct}, where we require the hypothesis to be exact in the $\rho$-balls around a point.

\begin{proposition} 
\label{prop:robust-loss-threshold-1}
For any probability measure $\mu$ on $\boolhc$, robustness parameter $\rho$ and concepts $h,c$, there exists $\epsilon>0$ such that if $\roblosse(h,c)<\epsilon$ then $h(x)=c(x)$ for any $x\in\X$ such that $\mu(B_\rho(x))>0$.
In particular, one has that $h$ and $c$ agree on the support of $\mu$.
\end{proposition}
\begin{proof}
Suppose there exists $x^*\in\X$ with $\mu(B_\rho(x^*))>0$ such that $h(x^*)\neq c(x^*)$. 
Then for any $z\in B_\rho(x^*)$, we have that $\roblosse(h,c,z)$, the robust loss of $h$ with respect to $c$ at point $z$, is 1.
Let $\tilde{\X}:=\set{x\in\X:\mu\left(B_\rho(x)\right)>0}$, and  $\epsilon=\min_{x\in\tilde{\X}}\mu(B_\rho(x))$. 
We have that
\begin{align*}
\roblosse(h,c)
&\geq\sum_{z\in B_\rho(x^*)}\mu(\set{z})\ell_\rho^R(h,c,z)
=\mu(B_\rho(x^*))
\geq\epsilon
\enspace.
\end{align*} 
\end{proof}

\begin{corollary}
\label{cor:robust-to-exact-1}
For any fixed distribution $D$, robust learning with respect to $D$ implies distribution-specific exact learning with respect to $D$ for any robustness parameter as long as $\epsilon$ in Proposition~\ref{prop:robust-loss-threshold-1} satisfies $\epsilon^{-1}=\poly(n)$.
\end{corollary}

\begin{proof}
Fix a distribution $D\in\D$ on $\X$. 
Suppose that we have a $\rho$-robust learning algorithm $\A_\F^R(D)$ for $\F$, namely for all $\epsilon,\delta,\rho>0$, for all $c\in\F$, if $\A_\F^R(D)$ has access to a sample $S$ of size $m\geq \poly(\frac{1}{\epsilon},\frac{1}{\delta},\text{size}(c),d)$, it returns $f\in\F$ such that 
\begin{equation}
\Pr{S\sim D^m}{\ell_\rho^R(f,c)<\epsilon}\geq 1-\delta
\enspace.
\end{equation}

By Proposition~\ref{prop:robust-loss-threshold-1}, we can choose $\epsilon$ such that $\roblosse(h,c)<\epsilon$ implies that $h(x)=c(x)$ for any $x\in\X$ such that $\mu(B_\rho(x))>0$. 
Note that this $\epsilon$ depends on $D$, $\rho$ and $n$.
So we have that 

\begin{equation}
\Pr{x\sim D}{f(x)\neq c(x)}=0
\enspace,
\end{equation}
with probability at least $1-\delta$ over the training sample $S$, whose size remains polynomial in $\frac{1}{\delta}$ and $n$ by the theorem assumptions.
\end{proof}

\begin{remark}
The assumption on  $\epsilon$ in Corollary~\ref{cor:robust-to-exact-1} is necessary to use the robust learning algorithm as a black box: in Section~\ref{sec:rob-learning-unif}, we work under a well-behaved class of distributions that includes the uniform distribution and show that, for long enough monotone conjunctions and small enough robustness parameter (with respect to the conjunction length), efficient robust learning is possible.
However, we cannot exactly learn these monotone conjunctions.
In the uniform distribution setting, the $\rho$-balls all have the same probability mass and $\epsilon^{-1}$ is essentially exponential in $n$. 
Note that in the case of Section~\ref{sec:rob-learning-unif}, the robust learning algorithm is an exact learning algorithm by design, and $\epsilon^{-1}$ is polynomial in $n$.
\end{remark}

To show the same result  for $\roblossc$, where the hypothesis is constant in a ball, we can use the exact same reasoning as in Corollary~\ref{cor:robust-to-exact-1}, except that we need to show the analogue of Proposition~\ref{prop:robust-loss-threshold-1} for this setting.

\begin{proposition}
For any probability measure $\mu$ on $\boolhc$ and for any concepts $h,c$, there exists $\epsilon>0$ such that if $\roblossc(h,c)<\epsilon$ then $h$ and $c$ agree on the support of $\mu$.
\end{proposition}

\begin{proof}
Fix $h,c,D$ and let $\epsilon=\min_{x\in\supp(\mu)}\mu(\set{x})$.
Suppose there exists $x^*\in\supp(\mu)$ and $z\in B_\rho(x^*)$ such that $c(x^*)\neq h(z)$. Then
\begin{equation*}
\roblossc(h,c)
=\Pr{x\sim \mu}{\exists z\in B_\rho(x)\;.\; c(x)\neq h(z)}
\geq\epsilon
\enspace.
\end{equation*}
\end{proof}

*To check: Gap between the two definitions of epsilon: for the other definition, there is no "saving grace" from the robustness parameter, only the distribution matters.

